Connecting Deep-Reinforcement-Learning-based Obstacle Avoidance with Conventional Global Planners using Waypoint Generators

Deep Reinforcement Learning has emerged as an efficient dynamic obstacle avoidance method in highly dynamic environments. It has the potential to replace overly conservative or inefficient navigation approaches. However, the integration of Deep Reinforcement Learning into existing navigation systems is still an open frontier due to the myopic nature of Deep-Reinforcement-Learning-based navigation, which hinders its widespread integration into current navigation systems. In this paper, we propose the concept of an intermediate planner to interconnect novel Deep-Reinforcement-Learning-based obstacle avoidance with conventional global planning methods using waypoint generation. Therefore, we integrate different waypoint generators into existing navigation systems and compare the joint system against traditional ones. We found an increased performance in terms of safety, efficiency and path smoothness especially in highly dynamic environments.

==> content/acknowledgment.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex



==> content/keywords.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex


%\begin{IEEEkeywords}
%	Virtual Reality and Interfaces, Localization, Object Detection, Computer Vision for Other %Robotic Applications, AI-Based Methods
%\end{IEEEkeywords}

==> content/title.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex

%\title{A robust pose estimator for articualted robots using monocular cameras and Deep-Learning-based keypoint detection\\
%	}
%	\thanks{Identify applicable funding agency here. If none, delete this.}
%}
\title{\LARGE \bf
Towards Augmented Reality Simulation in Robotics - Facing Barriers of Industrial Applicability
}

\author{Jens Lambrecht$^{1}$, Linh Kästner$^{1}$, Jan Guhl$^{2}$ and J\"org Kr\"uger$^{2}$% <-this % stops a space% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Jens Lambrecht and Linh Kästner are with the Chair Industry Grade Networks and Clouds, Faculty of Electrical Engineering and Computer Science,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small lambrecht@tu-berlin.de}}%
\thanks{$^{2}$Jan Guhl and J\"org Kr\"uger are with the Chair Industrial Automation Technology, Faculty of Mechanical Engineering and Transport Systems,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small guhl@iat.tu-berlin.de}}%        
}


%\author{
%	\IEEEauthorblockN{Jens Lambrecht}
%	\IEEEauthorblockA{\textit{Chair Industry Grade Networks and Clouds} \\
%		\textit{Technische Universität Berlin}\\
%		Berlin, Germany \\
%		lambrecht@tu-berlin.de}
%}

\maketitle
